Mixed Sessions: the Other Side of the Tape

The original paper on Mixed Sessions introduce the side A of the tape: there is an encoding of classical sessions into mixed sessions. Here we present side B: there is a translation of (a subset of) mixed sessions into classical session types. We prove that the translation is a minimal encoding, according to the criteria put forward by Kouzapas, P\'erez, and Yoshida.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{S. Balzer, L. Padovani (Eds.): Programming Language Approaches\\
to Concurrency- \& Communication-cEntric Software (PLACES 2020)\\
EPTCS 314, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.314.5}{10.4204/EPTCS.314.5}}

